Explicit Box Detection Unifies End-to-End Multi-Person Pose Estimation

This paper presents a novel end-to-end framework with Explicit box Detection for multi-person Pose estimation, called ED-Pose, where it unifies the contextual learning between human-level (global) and keypoint-level (local) information. Different from previous one-stage methods, ED-Pose re-considers this task as two explicit box detection processes with a unified representation and regression supervision. First, we introduce a human detection decoder from encoded tokens to extract global features. It can provide a good initialization for the latter keypoint detection, making the training process converge fast. Second, to bring in contextual information near keypoints, we regard pose estimation as a keypoint box detection problem to learn both box positions and contents for each keypoint. A human-to-keypoint detection decoder adopts an interactive learning strategy between human and keypoint features to further enhance global and local feature aggregation. In general, ED-Pose is conceptually simple without post-processing and dense heatmap supervision. It demonstrates its effectiveness and efficiency compared with both two-stage and one-stage methods. Notably, explicit box detection boosts the pose estimation performance by 4.5 AP on COCO and 9.9 AP on CrowdPose. For the first time, as a fully end-to-end framework with a L1 regression loss, ED-Pose surpasses heatmap-based Top-down methods under the same backbone by 1.2 AP on COCO and achieves the state-of-the-art with 76.6 AP on CrowdPose without bells and whistles. Code is available at https://github.com/IDEA-Research/ED-Pose.

==> sec/TODO.tex <==
实验（待做）：
1、单独训练检测（medium, large）(2层以及4层)
2、Label Task
3、Inferene time (EP-Pose）V100
4、R50 test-dev
5、box-keypoint decoder layer
6、no mask 
7、multi-scale flip nms

实验（进行中）：
1、无box loss >> 引入box detection的好处
2、无box kypoint交互 >> 引入interactive learning的好处
3、vit-h/vitpose-h大模型


实验（done）:
1、keypoint hw的4D表征
2、R50 val
3、SwinL val/test-dev
4、queries number
5、

